Blowing cold flows away: the impact of early AGN activity on the formation of a brightest cluster galaxy progenitor

Supermassive black holes (BH) are powerful sources of energy that are already in place at very early epochs of the Universe (by z=6). Using hydrodynamical simulations of the formation of a massive M_vir=5 10^11 M_sun halo by z=6 (the most massive progenitor of a cluster of M_vir=2 10^15 M_sun at z=0), we evaluate the impact of Active Galactic Nuclei (AGN) on galaxy mass content, BH self-regulation, and gas distribution inside this massive halo. We find that SN feedback has a marginal influence on the stellar structure, and no influence on the mass distribution on large scales. In contrast, AGN feedback alone is able to significantly alter the stellar-bulge mass content by quenching star formation when the BH is self-regulating, and by depleting the cold gas reservoir in the centre of the galaxy. The growth of the BH proceeds first by a rapid Eddington-limited period fed by direct cold filamentary infall. When the energy delivered by the AGN is sufficiently large to unbind the cold gas of the bulge, the accretion of gas onto the BH is maintained both by smooth gas inflow and clump migration through the galactic disc triggered by merger-induced torques. The feedback from the AGN has also a severe consequence on the baryon mass content within the halo, producing large-scale hot superwinds, able to blow away some of the cold filamentary material from the centre and reduce the baryon fraction by more than 30 per cent within the halo's virial radius. Thus in the very young universe, AGN feedback is likely to be a key process, shaping the properties of the most massive galaxies.

==> PaxHeader/BHfeed.tex <==
17 gid=589157795
18 uid=1219262348
20 ctime=1350301712
20 atime=1350303097
38 LIBARCHIVE.creationtime=1346148875
24 SCHILY.dev=234881026
22 SCHILY.ino=4475605
18 SCHILY.nlink=1

